Taylor Videos for Action Recognition

Effectively extracting motions from video is a critical and long-standing problem for action recognition. This problem is very challenging because motions (i) do not have an explicit form, (ii) have various concepts such as displacement, velocity, and acceleration, and (iii) often contain noise caused by unstable pixels. Addressing these challenges, we propose the Taylor video, a new video format that highlights the dominate motions (e.g., a waving hand) in each of its frames named the Taylor frame. Taylor video is named after Taylor series, which approximates a function at a given point using important terms. In the scenario of videos, we define an implicit motion-extraction function which aims to extract motions from video temporal block. In this block, using the frames, the difference frames, and higher-order difference frames, we perform Taylor expansion to approximate this function at the starting frame. We show the summation of the higher-order terms in the Taylor series gives us dominant motion patterns, where static objects, small and unstable motions are removed. Experimentally we show that Taylor videos are effective inputs to popular architectures including 2D CNNs, 3D CNNs, and transformers. When used individually, Taylor videos yield competitive action recognition accuracy compared to RGB videos and optical flow. When fused with RGB or optical flow videos, further accuracy improvement is achieved. Additionally, we apply Taylor video computation to human skeleton sequences, resulting in Taylor skeleton sequences that outperform the use of original skeletons for skeleton-based action recognition.

==> backup.tex <==

\section{Related Work}

\noindent\textbf{Conventional RGB videos.}
% A conventional RGB video is constructed as a sequence of individual RGB frames, each frame being a single RGB image. This main premise of 
Conventional RGB videos are constructed by sequencing multiple RGB images / frames. RGB videos fundamentally lack in temporal representations, due to no temporal information being present in its individual frames. For models to distill temporal knowledge from RGB videos, architectural change is needed, which leads to more advanced architectures, but these improved architectures often require substantially more resources to train and test. 

A considerable amount of redundant information is also present within RGB videos. Since motion is only stored in a fractional amount in an RGB video, the other information within RGB videos are not necessary for model learning. Optic flow's improvement to action recognition performance whilst eliminating RGB format's noisy information is evidence to this. 

In 2016, Wang et al. introduced TSN, a 2D convolutional network architecture deliberately structured to account for long term temporal learning. This work made evident that improving temporal understanding in models would additionally improve its performance. 3D convolutional networks such as Carreira and Zisserman's I3D altered network modality, such that compared to their 2D counterparts, these 3D networks don't pass in RGB videos to models frame by frame, instead, multiple frames are fed simultaneously. This form of 3D network design provide enhanced temporal learning than 2D networks, as well as better overall performance. But 3D networks achieve this by having larger and more complex architectures, as a result, they are more computationally intensive to train and test than 2D networks. This motivated Lin et al.'s work of the TSM architecture, an improved 2D network based on TSN. TSM's architecture retains TSN's 2D network complexity, but enjoys the increased temporal learning of a 3D network like I3D. However, the temporal learning improvement provided is still limited, as well as the fact that TSM and other previously mentioned models are all RGB based architectures, meaning they extract unusable spatial-temporal features from RGB video's large amounts of redundant information.

At present, large language models (LLMs) for action recognition are rising in popularity due to their high performance. These LLMs use powerful, RGB pre-trained transformer models(\eg VideoMAEv2, TimeSformer, etc.) to achieve the best results. While these transformer models are incredibly strong, they still suffer limitations similar to 2D and 3D networks. Wang et al.'s VideoMAEv2 utilizes an auto masked encoder to mask out regions within the inputs (RGB videos), and compels the model to learn to recover the originally masked out information. Like the 2D and 3D networks, VideoMAEv2's performance suffers from RGB video's nature of storing large amounts of redundant spatial information. The intensive process of masked auto encoding wastes a great amount of resources teaching the model to recover useless and redundant information. Transformers that uses patching such as Bertasius et al.'s TimeSformer model suffer a similar issue. When patching is applied to RGB video data, a number of the patches wouldn't contain motion information at all, meaning that the transformers will be distilling spatial-temporal features from the redundant information in the RGB videos, which wastes calculation resources, elongates learning time and limits performance. 

Our Taylor videos are able to resolve all the issues mentioned above, as in comparison to RGB videos, our method is able to represent spatial-temporal information of motions in a much more concise, light-weight and accurate manner. The improved temporal representation our method provides grants easier temporal learning for different architecture types. Our method also eliminates all the redundant information present in RGB videos, as well as highlight the dominant motions, so that only the necessary motion information is passed into the model to learn. In these ways, our method is able to boost the performance of RGB architectures of different types, without altering their architecture, and only changing the input data.

\noindent\textbf{Optical flow videos.}
Optical flow estimation methods calculate vectors that represent motions of individual pixels. Compared to RGB representation, optical flow is able to eliminate a sizeable portion of redundant spatial information, as well as include a pre-determined amount of temporal information in its frames. 

The various optical flow estimation methods use either traditional handcrafted methods, or machine learning based methods. Handcrafted methods generally provide accurate and strong short-term temporal representations (i.e. LDOF), but most handcrafted methods (e.g. LDOF, DeepFlow, etc.) can not outperform machine learning based methods (e.g. UnFlow, GMFlow)in long-term temporal representations. However, state-of-the-art for both methodologies require significant amount of resources to calculate. Optic flow is also unable to accurately capture both short term and long term temporal information, and have difficulty representing motions accurately in certain scenarios (i.e. fast movements, noise from source videos). These optical flow methods also capture noisy residual motions, as they are unable to isolate our the dominant motions in a video. 

% Optical flow is often used in multi-stream architectures rather than single stream, as optical flow complements in RGB for action recognition performance. These architectures (i.e. I3D) that utilize optical flow as one of its streams are able to get state-of-the-art results across popular action recognition data sets. 

Compared to optical flow, Taylor videos are able to more consistently, accurately and deliberately represent motion information. Taylor videos accurately captures both short-term and long-term temporal information. Additionally, our method highlights the dominant motions, and is able to recover residual motions using more terms of the Taylor approximation series, while optical flow estimations can not filter out the noisy residual motions. Optical flow represents videos with two channels, while traditional RGB and Taylor videos use three, hence architectural change is required to train and test on optical flow, while our method can directly be fed as data into models designed for conventional RGB representation.

\noindent\textbf{Forming short-term motions in a single frame.}
Kiyoon et al. introduced a channel sampling method to assist models perform temporal learning without architecture change. The method involves stacking consecutive frame's individual RGB channels together to form one single frame. This is able to better represent temporal information and lead to overall performance increase, however, this method is flawed in that it abandons information with its calculations. This method also isn't mathematically founded, as different frames in this method stack differently. 

In comparison, Taylor videos are able to help achieve better temporal learning than the channel sampling method, and uses well-founded mathematical concepts to build the representation. Our method is also able to eliminate redundant information of RGB videos while the channel sampling method is unable to.
